Granular mixing and flow dynamics in horizontal stirred bed reactors

Horizontal stirred bed reactors (HSBRs) are used in gas--phase polyolefin production, where efficient solids mixing and controlled residence time distributions are essential for product quality and stability. Despite their industrial relevance, the influence of operating conditions on granular flow and mixing in HSBRs is not well understood. Discrete Element Method (DEM) simulations are used to study the effects of rotation speed and fill level on particle motion, mixing, and axial transport in a lab--scale HSBR. An industrial--grade polypropylene powder is modelled using calibrated contact parameters. Mixing is quantified using the Lacey index in axial (z) and cross--sectional (xy) directions. Particle circulation is characterised via cycle--time analysis and a coarse--grained angular velocity field. Axial dispersion coefficients are obtained from particle trajectories using both Einstein--type and cycle--based approaches, and validated with a diffusion model predicting the axial Lacey index. Results show that axial mixing depends strongly on rotation speed and fill level: higher rotation speeds accelerate homogenization, while higher fill levels slow mixing. Cross--sectional mixing is mainly sensitive to rotation speed, with fill--level effects diminishing at higher speeds. Cycle time decreases with increasing rotation speed and fill level, indicating enhanced circulation. Axial dispersion increases with rotation speed but decreases with fill level, with consistent results across methods. These findings reveal trade--offs between axial mixing, circulation, and dispersion, highlighting the need to balance operating conditions and demonstrating the capability of DEM to support HSBR optimisation.

==> PreExp.tex <==
%
\textcolor{blue}{A calibration of the DPM model parameters is required to accurately predict the bulk behaviour of a powder material. Here, we have not attempted to match the rolling, sliding friction coefficients and surface energy to any specific Ti-6Al-4V powder material. The current work's aim is to show the qualitative effect of those parameters on the powder layer quality. 
%Nevertheless, some parameter combinations do represent real materials, as discussed here.
For an accurate calibration, the particle and contact properties should be chosen to match the static and dynamic angle of repose, the cohesive strength, and the apparent density of the powder material -- all tests under low confining stress \cite{Shi2020}, 
% SL if you agree, pls add Haos paper with Lumay, and dont we have another paper with calibration?
as relevant for powder spreading. Note that the calibration can be done efficiently by taking advantage of a Bayesian calibration procedure \cite{Cheng2019}.}

\textcolor{blue}{So far, we have performed only one preliminary calibration measurement: we have simulated a static angle of repose (AOR) test, calculated the AOR, similar to Meier et al.\ \cite{Meier2019a} and compared the results to experimental AOR values of Ti-6Al-4V powder material. The simulation setup for measuring the AOR is illustrated in Fig.\,\ref{fig:funnelSetup}. The opening diameter was set to 0.4\,mm and the side length of the square base was set to 1.25\,mm. Meier et al.\ \cite{Meier2019a} and Han et al.\ \cite{Han2019} show that the size of the base has only little influence on the measured AOR. For some cases (mostly high frictional) of weakly cohesive particles ($Bo_\mathrm{50} = 4$), particles did not flow through the 0.4\,mm opening, so a larger one of 0.8\,mm is used. As most cases of strongly cohesive particles ($Bo_\mathrm{50} = 15$) did not flow through either the 0.4\,mm and 0.8\,mm openings,  1\,mm one is used instead. However, the highly frictional and strongly cohesive ones did not flow even at 1\,mm opening.
Figs.\,\ref{fig:AORall}a, \ref{fig:AORall}b and \ref{fig:AORall}c show the numerically measured AOR for $Bo_\mathrm{50} =$ 0, 4 and 15, respectively. We see that the AOR increases as interparticle friction and cohesion increase. The white space in Fig.\,\ref{fig:AORall}c indicates no-flow.}

\textcolor{blue}{Meier et al.\ \cite{Meier2019a} measured the static angle of repose (AOR) of Ti-6Al-4V powder material for calibration. They have focused on the cohesion effect in terms of the effective surface energy, ignoring the effect of rolling resistance, only considered rolling dissipation and particle sizes between $D_\mathrm{10}$ and $D_\mathrm{90}$ i.e.\ low polydispersity. Following the same approach for measuring the AOR, including interparticle rolling friction and high polydispersity, we obtain a qualitative comparison with their results. They have found that the AOR is approximately $41\,^{\circ}$ with $\mu_\mathrm{s} = 0.4$ and $\gamma = 0.1\,\mathrm{mJ/m^{2}}$ matches the experimentally measured AOR. This corresponds to our results for the same parameters with approximately $\mu_\mathrm{r} = 0.05$, the red circle in Fig.\,\ref{fig:AORall}b. A top view snapshot of the powder layers with $\mu_\mathrm{s} = 0.4$, $\mu_\mathrm{r} = 0.05$ and $Bo_\mathrm{50} =$ 0, 4 and 15 are illustrated in Figs.\,\ref{fig:refToMeier}a, \ref{fig:refToMeier}b and \ref{fig:refToMeier}c, respectively. These snapshots show that the results are qualitatively comparable with Meire et al.\ Figs.\,8e, 8g and 8h, respectively, \cite{Meier2019b}.}
%
\textcolor{blue}{In addition, we have measured the AOR of another Ti-6Al-4V powder material with same PSD used in our simulations, relatively spherical particles shape and some satellite particles \cite{cordova2020}. We find that the average measured value of AOR is approximately $44\,^{\circ}$, Fig.\,\ref{fig:measuredAOR}.
%SEM images of the powder are available in \cite{cordova2020}. 
If we assume that the surface energy $\gamma = 0.1\,\mathrm{mJ/m^{2}}$ and small rolling friction $\mu_\mathrm{r} = 0.05$ (since the particles are relatively spherical) then the corresponding sliding friction $\mu_\mathrm{s}$ is between 0.5 and 0.2, Fig.\,\ref{fig:AORall}b.}

\textcolor{red}{This way we have provided a basic (rough) calibration with two reference Ti-6Al-4V powder materials. We then investigate how the changes in the powder material characteristics will influence the powder layer quality, by varying the values of interparticle friction and cohesion as presented in section \ref{sec:DOS}. Which is one of the main objectives of this paper.
It should be noted that} \textcolor{blue}{AOR is usually used for calibration and powder flowability assessment. However, It is not a sufficient or stand-alone measure. Powder flowability is one of the terms used to determine powder quality. Although this does not relate directly to powder ``spreadability''. We discuss further powder ``spreadability'' assessment and present a simple verification in section \ref{sec:exp2}} 
% SL I propose to remove
%\textcolor{red}{qualitative} 
%\footnote{YS: should I move the following to separate subsection in the results?}
%Recently, Cordova et al.\ \cite{cordova2020} have used two wiper blades ``applicator tools'' designed by the Netherlands Aerospace Centre (NLR) to manually access powder ``spreadability'' for the applications in LPBF. Both tools have the same blade profile. The first one ``open tool'' spread the powder avalanche directly over a metal strip, while in the second tool ``funnel tool'' the powder is spread through a funnel like shape. They have quantified a thin layer ($100\,\mathrm{\mu m}$) quality  of four different powders and concluded that the ``open tool'' is better to access the ``spreadability'' of moisturised powder. Another study by Ahmed et al.\ \cite{ahmed2020simple} have used a simple method to investigate powder layer uniformity. They have spread a powder layer manually over a glass slide covered by Emery paper. Here, we have also used a simple method to obtain a qualitative comparison of powder layer quality between a blade spreader and cc rotating roller: Powder samples of equal weight were prepared and placed in front of each tool, using a small container box to form an avalanche. Then the powder was spread manually over a paper tape. The powder used in both experiments has the same AOR as Ti-6Al-4V, with measured AOR\,$\approx 44\,^{\circ}$.
%Fig.\,\ref{fig:QExp} illustrates the design of those tools and the corresponding layers spread. We see that a cc rotating roller has produced a better quality layer than a blade, as our results in section \ref{sec:results} predict. Further experiments using same type powder materials with different characteristics will provide more qualitative and quantitative verification and validation.}


